Universal Semi-supervised Model Adaptation via Collaborative Consistency Training

In this paper, we introduce a realistic and challenging domain adaptation problem called Universal Semi-supervised Model Adaptation (USMA), which i) requires only a pre-trained source model, ii) allows the source and target domain to have different label sets, i.e., they share a common label set and hold their own private label set, and iii) requires only a few labeled samples in each class of the target domain. To address USMA, we propose a collaborative consistency training framework that regularizes the prediction consistency between two models, i.e., a pre-trained source model and its variant pre-trained with target data only, and combines their complementary strengths to learn a more powerful model. The rationale of our framework stems from the observation that the source model performs better on common categories than the target-only model, while on target-private categories, the target-only model performs better. We also propose a two-perspective, i.e., sample-wise and class-wise, consistency regularization to improve the training. Experimental results demonstrate the effectiveness of our method on several benchmark datasets.

==> latex/sup_misc/3_shot_domainnet.tex <==
\begin{table*}[t]
    \centering
    \caption{H-score on \textit{Domainnet} under the settings of 3-shot using ResNet34 as the backbone.}
    \setlength\tabcolsep{3pt}
    \scalebox{1}{
        \begin{tabular}{l|ccccccc}
        \toprule
        \textbf{Method}
        &  R $\rightarrow$ C
        &  P $\rightarrow$ C
        &  C $\rightarrow$ S
        &  R $\rightarrow$ P
        &  S $\rightarrow$ P
        &  R $\rightarrow$ S
        & \textbf{Mean} \\  
        \midrule
        CE       & 50.8 & 53   & 47.1 & 50.3 & 53.5 & 43.6 & 49.7 \\
        ENT      & 45.9 & 44.3 & 36.0 & 36.8 & 43.0 & 36.3 & 40.4 \\
        MixMatch & 48.0 & 50.5 & 44.4 & 50.1 & 50.2 & 44.2 & 47.9 \\
        FixMatch & 52.5 & 48.2 & 49.8 & 52.8 & 48.6 & 43.0 & 49.2 \\
        UMA      & 42.7 & 46.2 & 41.7 & 42.9 & 40.4 & 40.2 & 42.3 \\
        MME      & 56.7 & 58.9 & 45.0 & 49.9 & 52.7 & 42.8 & 51.0 \\
        CDAC     & 59.0 & 59.2 & 50.8 & 62.3 & 62.3 & 51.9 & 57.6 \\
        SSHT     & 64.1 & 66.8 & 54.2 & 59.0 & 65.6 & 47.1 & 59.5 \\
        SHOT++   & 55.6 & 59.4 & 51.0 & 56.1 & 56.7 & 45.4 & 54.0 \\
        CCT      & \textbf{69.9} & \textbf{69.0} & \textbf{58.6} & \textbf{66.7} & \textbf{67.4} & \textbf{56.2} & \textbf{64.6} \\
        \bottomrule
        \end{tabular}
    }
    \label{table:3shot_domainnet}
\end{table*}

==> latex/sup_misc/3_shot_officehome.tex <==
\begin{table*}[t]
    \centering
    \caption{ H-score on \textit{Office-Home} under the settings of 3-shot using ResNet34 as the backbone.}
    \setlength\tabcolsep{2.1pt}
    \scalebox{1}{
        \begin{tabular}{l|ccccccccccccc}
        \toprule
        \textbf{Method}
        & \small A $\rightarrow$ C
        & \small A $\rightarrow$ P
        & \small A $\rightarrow$ R
        & \small C $\rightarrow$ A
        & \small C $\rightarrow$ P
        & \small C $\rightarrow$ R
        & \small P $\rightarrow$ A
        & \small P $\rightarrow$ C
        & \small P $\rightarrow$ R
        & \small R $\rightarrow$ A
        & \small R $\rightarrow$ C
        & \small R $\rightarrow$ P
        & \textbf{Mean} \\  
        \midrule
        CE       & 51.8 & 73.9 & 69.9 & 49.9 & 70.7 & 65.6 & 57.8 & 51.1 & 68.9 & 55.7 & 54.0 & 74.6 & 62.0 \\
        ENT      & 53.2 & 76.4 & 71.7 & 46.3 & 74.9 & 66.1 & 54.6 & 46.5 & 69.4 & 57.3 & 54.8 & 77.2 & 62.4 \\
        MixMatch & 51.3 & 77.6 & 73.3 & 51.8 & 76.4 & 69.7 & 56.8 & 51.1 & 72.2 & 58.3 & 53.4 & 78.5 & 64.2 \\
        FixMatch & 50.6 & 76.2 & 67.5 & 39.9 & 76.6 & 66.9 & 53.9 & 56.7 & 67.4 & 47.1 & 51.8 & 75.4 & 60.8 \\
        UMA     & 54.6 & 76.3 & 71.3 & 52.1 & 73.7 & 63.3 & 57.2 & 52.5 & 68.8 & 54.0 & 56.4 & 76.2 & 63.0 \\
        MME      & 55.6 & 77.1 & 72.3 & 55.2 & 75.3 & 68.8 & 60.0 & 53.6 & 72.5 & 61.4 & 57.8 & 77.3 & 65.6 \\
        CDAC     & 55.7 & 76.3 & 72.0 & 54.0 & 75.4 & 68.9 & 54.5 & 58.8 & 72.3 & 60.6 & 57.1 & 76.9 & 65.2 \\
        SSHT     & 55.0 & 73.0 & 69.9 & 56.0 & 72.3 & 67.0 & 51.4 & 53.9 & 68.6 & 58.0 & 59.1 & 74.0 & 63.2 \\
        SHOT++   & 54.9 & 80.3 & 74.2 & 53.3 & 73.9 & 70.8 & 55.9 & 52.3 & 76.9 & 50.2 & 52.7 & 79.3 & 64.6 \\
        CCT     & \textbf{57.8} & \textbf{80.6} & \textbf{77.3} & \textbf{61.0} & \textbf{79.4} & \textbf{76.9} & \textbf{62.6} & \textbf{57.8} & \textbf{77.1} & \textbf{63.4} & \textbf{59.2} & \textbf{80.2} & \textbf{69.4} \\
        \bottomrule
        \end{tabular}
    }
    \label{table:3shot_office_home}
\end{table*}

==> latex/sup_misc/alg.tex <==
\begin{algorithm}[t]
\caption{Pseudocode of CCT in a PyTorch-like style.}
\label{alg:code}
\definecolor{codeblue}{rgb}{0.25,0.5,0.5}
\lstset{
  backgroundcolor=\color{white},
  basicstyle=\fontsize{7.2pt}{7.2pt}\ttfamily\selectfont,
  columns=fullflexible,
  breaklines=true,
  captionpos=b,
  commentstyle=\fontsize{7.2pt}{7.2pt}\color{codeblue},
  keywordstyle=\fontsize{7.2pt}{7.2pt},
%  frame=tb,
}
\begin{lstlisting}[language=python]
# f_1, f_2: source and target network
# T: threshold
# @: matrix multiplication
# lambda: loss weight for class-wise consistency

def sample_wise(p_1, p_2):
    max_probs, y = p_1.max(dim=1)
    mask = max_probs.ge(T).float() # thresholding 
    loss = CE(p_2, y, reduction='none') * mask
    return loss.mean()

def class_wise(p_1, p_2):
    N, C = p_1.shape
    corr = p_1.t() @ p_2 # C by C
    corr = (corr + corr.t()) / 2  # symmetrization
    corr = corr / corr.sum(dim=0) # normalization
    loss = -corr.trace() / C
    return loss

# load a minibatch x with N samples
for i_step in range(num_steps):
    x, y = loader_x.next() # labeled samples
    x_u = loader_x_u.next() # unlabeled samples
    
    x_1, x_2 = aug_1(x_u), aug_2(x_u) # augmentations
    
    Ps, Pt = f_s(x), f_t(x) # softmax predictions
    Ps_1, Ps_2 = f_s(x_1), f_s(x_2)
    Pt_1, Pt_2 = f_t(x_1), f_t(x_2)
    
    Lx = CE(Ps, y) + CE(Pt, y) # loss of labeled samples
    
    # sample-wise consistency loss
    L_sample = sample_wise(Ps_1, Ps_2)
               + sample_wise(Pt_1, Ps_2)
               + sample_wise(Ps_1, Pt_2)
               + sample_wise(Pt_1, Pt_2)
    
    # class-wise consistency loss
    L_class = class_wise(Ps_1, Ps_2)
               + class_wise(Pt_1, Ps_2)
               + class_wise(Ps_1, Pt_2)
               + class_wise(Pt_1, Pt_2)
    
    Loss = Lx + 0.5 * (L_sample + lambda * L_class)
    Loss.backward()
\end{lstlisting}
% \vspace{-4mm}
\end{algorithm}

==> latex/sup_misc/common_private_acc.tex <==
\begin{table*}[t]
    \centering
    \caption{ Accuracy of Common~($a_{\mathcal{C}}$) and Private~($a_{\mathcal{P}}$) set on the \textit{DomainNet} 5-shot setting using ResNet34 as the backbone.}
    \setlength\tabcolsep{8pt}
    \scalebox{0.8}{
        \begin{tabular}{l|cccccccccccccc}
        \toprule
        & \multicolumn{2}{c}{R $\rightarrow$ C} 
        & \multicolumn{2}{c}{P $\rightarrow$ C} 
        & \multicolumn{2}{c}{C $\rightarrow$ S}
        & \multicolumn{2}{c}{R $\rightarrow$ P} 
        & \multicolumn{2}{c}{S $\rightarrow$ P}
        & \multicolumn{2}{c}{R $\rightarrow$ S} 
        % & \multicolumn{2}{c|}{P $\rightarrow$ R}
        & \multicolumn{2}{c}{\textbf{Mean}} \\  
        \textbf{Method}
        & \small $a_{\mathcal{C}}$ & \small $a_{\mathcal{P}}$
        & \small $a_{\mathcal{C}}$ & \small $a_{\mathcal{P}}$
        & \small $a_{\mathcal{C}}$ & \small $a_{\mathcal{P}}$
        & \small $a_{\mathcal{C}}$ & \small $a_{\mathcal{P}}$
        & \small $a_{\mathcal{C}}$ & \small $a_{\mathcal{P}}$
        & \small $a_{\mathcal{C}}$ & \small $a_{\mathcal{P}}$
        % & \small 1-shot & \small Private
        & \small \textbf{$a_{\mathcal{C}}$} & \small \textbf{$a_{\mathcal{P}}$}\\
        \midrule
       CE       & 73.6 & 47.9 & 72.2 & 47.4 & 65.5 & 46.8 & 67.3 & 50.4 & 67.3 & 51.4 & 65.0 & 41.4 & 68.5 & 47.6 \\
        MME      & 74.8 & 59.8 & 73.7 & 56.7 & 62.4 & 49.5 & 63.1 & 61.6 & 65.8 & 61.9 & 62.4 & 43.4 & 67.0 & 55.5 \\
        FixMatch & 82.2 & 58.9 & 81.8 & 55.9 & 72.7 & 52.8 & 71.5 & 65.7 & 73.9 & 63.4 & 73.1 & 57.1 & 75.9 & 59.0 \\
        CCT      & \textbf{83.0} & \textbf{73.1} & \textbf{81.6} & \textbf{73.6} & \textbf{74.1} & \textbf{60.8} & \textbf{77.3} & \textbf{73.8} & \textbf{75.8} & \textbf{74.7} & \textbf{75.1} & \textbf{60.2} & \textbf{77.8} & \textbf{69.4} \\
        \bottomrule
        \end{tabular}
    }
    \label{table:Common_Private_acc}
\end{table*}

==> latex/sup_misc/comparion_officehome.tex <==
\begin{table}[t]
    \centering
    \caption{Average H-score on \textit{Office-Home} in the 3/5/10-shot settings using ResNet34 as the backbone.}
    \resizebox{0.85\linewidth}{!}{
        \begin{tabular}{
        p{2cm}|
        >{\centering\arraybackslash}p{1.5cm}
        >{\centering\arraybackslash}p{1.5cm}
        >{\centering\arraybackslash}p{1.5cm}
        }
        \toprule
        \textbf{Method}
        &  3-shot
        &  5-shot
        &  10-shot \\
        \midrule
        \multicolumn{4}{c}{Baselines}\\
        \midrule
        CE & 62.0 & 66.5 & 73.8 \\
        ENT & 62.4 & 70.0 & 77.5 \\
        \midrule
        \multicolumn{4}{c}{SSL methods}\\
        \midrule
        MixMatch & 64.2 & 70.2 & 77.5 \\
        FixMatch & 60.8 & 69.3 & 77.0 \\
        \midrule
        \multicolumn{4}{c}{SSDA methods}\\
        \midrule
        MME & 65.6 & 70.5 & 77.4 \\
        CDAC & 65.2 & 69.4 & 76.3 \\
        \midrule
        \multicolumn{4}{c}{SFSSDA methods}\\
        \midrule
        SSHT & 63.2 & 66.6 & 73.5 \\
        \midrule
        \multicolumn{4}{c}{USFDA methods}\\
        \midrule
        USFDA & 63.0 & 65.7 & 74.2 \\
        \midrule
        \midrule
        CCT & \textbf{69.4} & \textbf{73.5} & \textbf{78.7} \\
        \bottomrule
        \end{tabular}
    }
    \label{table:more_comparison_officehome}
\end{table}

==> latex/sup_misc/comparisons.tex <==
\begin{table}[t]
    \centering
    \caption{Average H-score on \textit{Domainnet} in the 3/5/10-shot settings using ResNet34 as the backbone.}
    \resizebox{0.85\linewidth}{!}{
        \begin{tabular}{
        p{2cm}|
        >{\centering\arraybackslash}p{1.5cm}
        >{\centering\arraybackslash}p{1.5cm}
        >{\centering\arraybackslash}p{1.5cm}
        }
        \toprule
        \textbf{Method}
        &  3-shot
        &  5-shot
        &  10-shot \\
        \midrule
        \multicolumn{4}{c}{Baselines}\\
        \midrule
        CE & 49.7 & 56.2 & 64.1 \\
        ENT & 40.0 & 55.1 & 69.7 \\
        \midrule
        \multicolumn{4}{c}{SSL methods}\\
        \midrule
        MixMatch & 47.9 & 62.8 & 70.6 \\
        FixMatch & 49.2 & 66.2 & 74.6 \\
        \midrule
        \multicolumn{4}{c}{SSDA methods}\\
        \midrule
        MME & 51.0 & 60.5 & 66.7 \\
        CDAC & 57.6 & 68.7 & 73.9 \\
        \midrule
        \multicolumn{4}{c}{SFSSDA methods}\\
        \midrule
        SSHT & 59.5 & 66.2 & 70.0 \\
        \midrule
        \multicolumn{4}{c}{USFDA methods}\\
        \midrule
        USFDA & 42.3 & 54.8 & 65.4 \\
        \midrule
        \midrule
        CCT & \textbf{64.6} & \textbf{73.3} & \textbf{76.6} \\
        \bottomrule
        \end{tabular}
    }
    \label{table:more_comparison}
\end{table}

==> latex/sup_misc/loss_weight.tex <==
\begin{table}[t]
    \centering
    \caption{Average H-score w.r.t. loss weight $\lambda_2$ on \textit{Office-Home} in the 5-shot setting. Note that $\lambda_1$ is fixed to 1.}
    \setlength\tabcolsep{5.5pt}
    \scalebox{0.85}{
        \begin{tabular}{l|cccc}
        \toprule
        % \multicolumn{4}{c}{Loss weight $\lambda_2$} \\
        $\lambda_2$ & 0 & 0.5 &  1 &  1.5 \\
        \midrule
        H-score & 70.5 & 73.5 & 73.3 & 72.6 \\
        \bottomrule
        \end{tabular}
    }
    \label{table:loss_weight}
\end{table}

==> latex/sup_misc/loss_weight_1.tex <==
\begin{table}[t]
    \centering
    \caption{(a) Average H-score w.r.t. loss weight $\lambda_1$ on the  \textit{Office-Home} 5-shot setting. Note that $\lambda_2$ is fixed to 0.5. (b) Average H-score w.r.t. loss weight $\lambda_2$ on the  \textit{Office-Home} 5-shot setting. Note that $\lambda_1$ is fixed to 1.}
    \begin{minipage}{0.49\textwidth}
            \centering
            \setlength\tabcolsep{5.5pt}
            \scalebox{0.8}{
                \begin{tabular}{l|cccc}
                \toprule
                $\lambda_1$ & 0 & 0.5 &  1 &  1.5 \\
                \midrule
                H-score & 72.3 & 73.5 & 73.5 & 72.8 \\
                \bottomrule
                \end{tabular}
            } \\ \vspace{1mm} (a) \vspace{1mm}
    \end{minipage}
    \begin{minipage}{.49\textwidth}
            \centering
            \setlength\tabcolsep{5.5pt}
            \scalebox{0.8}{
                \begin{tabular}{l|cccc}
                \toprule
                $\lambda_2$ & 0 & 0.5 &  1 &  1.5 \\
                \midrule
                H-score & 70.5 & 73.5 & 73.3 & 72.6 \\
                \bottomrule
                \end{tabular}
            }\\ \vspace{1mm}(b)
        % \end{table}
    \end{minipage}%
    \label{tab:lambda}
    \vspace{-2mm}
\end{table}

==> latex/sup_misc/mcc.tex <==
\begin{table}[t]
    \centering
    \setlength\tabcolsep{10pt}
    \caption{Comparison of class-wise consistency with MIM and MCC on \textit{Domainnet} 5-shot setting}
    \scalebox{0.8}{
        \begin{tabular}{l|cc}
        \toprule
        \textbf{Method}
         & R $\rightarrow$ C
        & C $\rightarrow$ S \\
        \midrule
        MIM & 55.2 & 51.0 \\
        MCC & 65.8 & 59.0 \\
        Class-wise~(ours) & \textbf{70.6} & \textbf{60.6} \\
        \midrule
        Sample-wise + MIM & 68.7 & 62.6 \\
        Sample-wise + MCC & 71.7 & 64.4 \\
        CCT~(ours) & \textbf{77.7} & \textbf{66.8} \\
        \bottomrule
        \end{tabular}
    }
    \label{table:comparison_mcc}
\end{table}

==> latex/sup_misc/multiple_run.tex <==
\begin{table}[t]
    \centering
    \caption{Mean and standard deviation of H-score over five runs on \textit{Domainnet} on the 5-shot setting. Note that \textbf{Avg} denotes the Mean and standard deviation of the mean H-score over five runs.}
    \setlength\tabcolsep{2.5pt}
    \scalebox{1}{
        \begin{tabular}{l|ccccccc}
        \toprule
        \small \textbf{Method}
        &  \small \rotatebox[origin=c]{0}{R $\rightarrow$ C}
        &  \small \rotatebox[origin=c]{0}{P $\rightarrow$ C}
        &  \small \rotatebox[origin=c]{0}{C $\rightarrow$ S}
        &  \small \rotatebox[origin=c]{0}{R $\rightarrow$ P}
        &  \small \rotatebox[origin=c]{0}{S $\rightarrow$ P}
        &  \small \rotatebox[origin=c]{0}{R $\rightarrow$ S}
        & \small \textbf{Avg} \\  
        \midrule
        Mean & 77.8 & 77.4 & 66.4 & 75.1 & 75.4 & 66.3 & 73.1 \\
        STD & 0.4 & 0.3 & 0.3 & 0.8 & 0.6 & 0.4 & 0.2 \\
        \bottomrule
        \end{tabular}
    }
    \label{table:multiple_run}
\end{table}

==> latex/sup_misc/pl.tex <==
\begin{table}[t]
    \centering
    % \vspace{-2mm}
    \caption{Results of different pseudo label generation strategies for sample-wise consistency on \textit{Domainnet}}
    \setlength\tabcolsep{10pt}
    \scalebox{0.8}{
        \begin{tabular}{l|cc}
        \toprule
        \textbf{Consistency Loss}
         & R $\rightarrow$ C
        & C $\rightarrow$ S \\
        \midrule
        Ensemble & 75.3 & 65.6 \\
        Weighted ensemble & 75.4 & 65.6 \\
        Sample-wise & \textbf{77.7} & \textbf{66.8}   \\
        \bottomrule
        \end{tabular}
    }
    \label{table:pl}
\end{table}

==> latex/sup_misc/result_F.tex <==
\begin{table}[t]
    \centering
    \caption{H-score on the \textit{Domainnet} 5-shot setting.}
    \setlength\tabcolsep{2.4pt}
    \scalebox{0.8}{
        \begin{tabular}{l|ccccccc}
        \toprule
        \small \textbf{Method}
        &  \small \rotatebox[origin=c]{0}{R $\rightarrow$ C}
        &  \small \rotatebox[origin=c]{0}{P $\rightarrow$ C}
        &  \small \rotatebox[origin=c]{0}{C $\rightarrow$ S}
        &  \small \rotatebox[origin=c]{0}{R $\rightarrow$ P}
        &  \small \rotatebox[origin=c]{0}{S $\rightarrow$ P}
        &  \small \rotatebox[origin=c]{0}{R $\rightarrow$ S}
        & \small \textbf{Mean} \\  
        \midrule
        $F(\cdot|\theta_s)$ & 77.7 & 77.4 & 66.8 & 75.5 & 75.3 & 66.9 & \textbf{73.3} \\
        $F(\cdot|\theta_t)$ & 77.9 & 77.4 & 66.7 & 75.5 & 75.1 & 66.8 & 73.2 \\
        \bottomrule
        \end{tabular}
    }
    \label{table:result_F}
\end{table}

==> latex/sup_misc/ssl.tex <==
\begin{table}[t]
    \centering
    \caption{H-score of R $\rightarrow$ P and S $\rightarrow$ P on \textit{Domainnet} 5 settings.}
    \setlength\tabcolsep{10pt}
    \scalebox{0.8}{
        \begin{tabular}{l|cc}
        \toprule
         \textbf{Method}
        &  { R $\rightarrow$ P} 
        &  { S $\rightarrow$ P} \\
        \midrule
        RotPred & 71.8 & 73.9 \\
        SCL+SimCLR & \textbf{75.5} & \textbf{75.3}  \\
        \bottomrule
        \end{tabular}
    }
    \label{table:ssl}
\end{table}

==> latex/sup_misc/tsne.tex <==
\begin{figure*}[t]
    \vspace{2mm}
    \centering
    \begin{minipage}{0.33\textwidth}
        % \label{fig:p_size}
        \centering
        \includegraphics[width=.99\linewidth]{latex/Figures/mme_tsne.pdf}\\
        (a) MME.
    \end{minipage}
    \begin{minipage}{.33\textwidth}
        \centering
        \includegraphics[width=.99\linewidth]{latex/Figures/fix_tsne.pdf}\\
        (b) FixMatch.
        % \label{fig:c_size}
        \end{minipage}%
    \begin{minipage}{.33\textwidth}
    \centering
        \includegraphics[width=.99\linewidth]{latex/Figures/cct_tsne.pdf}\\
        (c) CCT.
        % \label{fig:num_shot}
    \end{minipage}%
    \caption{TSNE~\cite{van2008tsne} visualization of the learned features of common~(top) and private~(bottom) sets samples respectively. We randomly sample 20 classes for both sets in task R $\rightarrow$ C on \textit{Domainnet}.}
    \label{fig:tsne}
    % \vspace{-2mm}
\end{figure*}

==> latex/tables/analysis_aug.tex <==
\begin{table}[t]
    \centering
    \caption{\textit{H-score} w.r.t. augmentation strategies in task R $\rightarrow$ C and R $\rightarrow$ S on \textit{Domainnet}.}
    % \vspace{2mm}
    \setlength\tabcolsep{10pt}
    \scalebox{0.8}{
        \begin{tabular}{cc|cc}
        \toprule
        $\mathbf{x}^{\prime}$
        & $\mathbf{x}^{\dprime}$
        & R $\rightarrow$ C
        & R $\rightarrow$ S \\
        \midrule
        Strong &  Strong & 75.6 & 62.1\\
        Strong &  Weak & 60.0 & 56.7 \\
        Weak &  Weak & 72.8 & 61.3 \\
        Weak &  Strong & \textbf{77.7} & \textbf{66.8} \\
        \bottomrule
        \end{tabular}
    }
    \label{table:augmentation}
    % \vspace{-2mm}
\end{table}

==> latex/tables/analysis_thres.tex <==
\begin{table}[t]
    \centering
    \caption{\textit{H-score} w.r.t. threshold $\tau$ in task R $\rightarrow$ C on \textit{Domainnet}.}
    % \vspace{2mm}
    \setlength\tabcolsep{10pt}
    \scalebox{0.8}{
        \begin{tabular}{c|ccccc}
        \toprule
        & \multicolumn{5}{c}{Threshold $\tau$} \\
        Method & \small 0.35 & \small0.5 & \small0.65 & \small0.8 & \small0.95 \\
        \midrule
        FixMatch & 66.9& 65.7& 67.9& 70.4& 68.6 \\
        CCT & \textbf{73.7} & \textbf{73.5} & \textbf{73.4} & \textbf{76.3} &  \textbf{77.7} \\
        \bottomrule
        \end{tabular}
    }
    \label{table:threshold}
    \vspace{-2mm}
\end{table}

==> latex/tables/multiple_run.tex <==
\begin{table}[t]
    \centering
    \caption{Mean and standard deviation of H-score over five runs on \textit{Domainnet} in the 5-shot setting. Note that \textbf{Avg} denotes the Mean and standard deviation of the mean H-score over five runs.}
    % \vspace{2mm}
    \setlength\tabcolsep{4pt}
    \scalebox{0.8}{
        \begin{tabular}{c|cccccc|c}
        \toprule
        \small \textbf{Method}
        &  \small \rotatebox[origin=c]{0}{R $\rightarrow$ C}
        &  \small \rotatebox[origin=c]{0}{P $\rightarrow$ C}
        &  \small \rotatebox[origin=c]{0}{C $\rightarrow$ S}
        &  \small \rotatebox[origin=c]{0}{R $\rightarrow$ P}
        &  \small \rotatebox[origin=c]{0}{S $\rightarrow$ P}
        &  \small \rotatebox[origin=c]{0}{R $\rightarrow$ S}
        & \small \textbf{Avg} \\  
        \midrule
        Mean & 77.8 & 77.4 & 66.4 & 75.1 & 75.4 & 66.3 & 73.1 \\
        STD & 0.4 & 0.3 & 0.3 & 0.8 & 0.6 & 0.4 & 0.2 \\
        \bottomrule
        \end{tabular}
    }
    \label{table:multiple_run}
    \vspace{-2mm}
\end{table}
